An O(N) distributed-memory parallel direct solver for planar integral equations

Boundary value problems involving elliptic PDEs such as the Laplace and the Helmholtz equations are ubiquitous in mathematical physics and engineering. Many such problems can be alternatively formulated as integral equations that are mathematically more tractable. However, an integral-equation formulation poses a significant computational challenge: solving large dense linear systems that arise upon discretization. In cases where iterative methods converge rapidly, existing methods that draw on fast summation schemes such as the Fast Multipole Method are highly efficient and well-established. More recently, linear complexity direct solvers that sidestep convergence issues by directly computing an invertible factorization have been developed. However, storage and computation costs are high, which limits their ability to solve large-scale problems in practice. In this work, we introduce a distributed-memory parallel algorithm based on an existing direct solver named ``strong recursive skeletonization factorization.'' Specifically, we apply low-rank compression to certain off-diagonal matrix blocks in a way that minimizes computation and data movement. Compared to iterative algorithms, our method is particularly suitable for problems involving ill-conditioned matrices or multiple right-hand sides. Large-scale numerical experiments are presented to show the performance of our Julia implementation.

==> parfactor_bak.tex <==
\begin{algorithm}
\caption{\texttt{parallel factorization}}
%\label{alg:FMM:Parallel}
\begin{algorithmic}[1]
\Require{Kernel function $K$, points $\X = \{x_i\}_{i=1}^N \in \mathbb{R}^{2}$.}
\Ensure Factorization in \cref{e:alg}.



\For{$l = L, L-1, \ldots, 1$} 
\State [All processors] factorize interior boxes.
\For {4 colors}
\State [Processors with color $i$] factorize boundary boxes.
\EndFor
\State [All processors] construct the coarse level.
\EndFor



%\EndFor
%\Statex
\State{$K = A$}
\State{$D_1 \leftarrow$ distributed array containing information regarding geometry of boxes}
\State{$D_2 \leftarrow$ distributed array containing skeleton/redundant point information}
\State{$D_3 \leftarrow$ distributed array containing any modification made to matrices}
\State{$D_4 \leftarrow$ distributed array containing block matrices used for solving the linear system}
\State{$D_5 \leftarrow$ distributed array containing the coordinate of the active set of points in the domain}

\For{$l = L, \ldots, 1$}

\For{$p$ = 1, \ldots, $T$ }
 \hfill\Comment{\cyan{// looping over each process, is done in parallel}}
\State{$B(l)_p \leftarrow$ number of boxes on level $l$ that belong to process $p$}
\State{\red{Consult $D_1$ for locations, then fetch data from other processes portion of $D_2$ using rpc call}}
\For{$i = 1, \ldots, B(l)_p$}
\If{$B_i$ is an interior box}
\State{perform low rank compression (ID) to $A_{\mathcal B_i, \mathcal F}$ to obtain the interpolation matrix $T$} 
\State{perform block elimination $K = LP^\top\hat K P L^\top$ } 
\State{update $D_2, D_3$}
\EndIf
\EndFor
\EndFor

\For{$c = 1, \ldots, 2^d$} \hfill\Comment{\cyan{//looping through each color, $d$ is the dimension of the problem}}
\For{processes $p$ that have the same color corresponding to $c$}
\State{$B(l)_p \leftarrow$ number of boxes on level $l$ that belong to process $p$}
\For{$i = 1, \ldots, B(l)_p$}
\If{$B_i$ is an boundary box}
\State{perform low rank compression (ID) to $A_{\mathcal B_i, \mathcal F}$ to obtain the interpolation matrix $T$} 
\State{perform block elimination $K = LP^\top\hat K P L^\top$ } 
\EndIf
\EndFor
\State{\red{update $D_2, D_3$, since $B_i$ is on boundary, inter-process communication may be necessary unlike the non boundary boxes}}
\EndFor

\EndFor

\State{\red{Rebuild $D_3$ for next level in parallel, (i.e.) reorganize matrices such as $X_{\mathcal N, \mathcal N}$ by collecting the interaction of children boxes and combining them}} 
\State{\red{Rebuild the $D_5$ for the next level by taking only the skeleton points (active points) from each box}}
\EndFor \\
\end{algorithmic}
\end{algorithm}



==> solve.tex <==
\begin{algorithm}
\caption{\texttt{sequential solve}}
\label{a:solve}
\begin{algorithmic}[1]
\Require{ Factorization in \cref{e:alg} and a given right-hand-side $b \in \mathbb{R}^N$}
\Ensure The (approximate) solution of \cref{e:axb}, which overwrites $b$.
%
\Statex
\For{$\ell = L, L-1, \ldots, 1$} \Comment{\hfill \cyan{// bottom-up sweep}}
\For{$i = 1, 2, \ldots, n_\ell$} \Comment{\hfill \cyan{// ordering used in the factorization}}
\State{ Update \emph{local} data $b(\R)$ and $b(\S)$ for box $\B_i$: 
%
\[
\begin{array}{ccr}
b(\R) & \mathrel{-}= &  T^\top \, b(\S) \\
b(\R) & = & L_{\R}^{-1} \, b(\R) \\
b(\S) & \mathrel{-}= & X_{\S, \R} U_{\R}^{-1} \, b(\R) \\
\end{array}
\]
} 
\Comment{\hfill \cyan{// $\R, \S$ and $T$ defined in \cref{e:t}; $L_{\R}$, $U_{\R}$, and $X_{\S, \R}$ defined in \cref{e:step} }}
%
\State{ Update \emph{neighbors'} data $b(\N)$ for box $\B_i$:
\[
\begin{array}{ccr}
b(\N) \mathrel{-}= X_{\N, \R} U_{\R}^{-1} \, b(\R)
\end{array}
\]
} 
\Comment{\hfill \cyan{// $X_{\N, \R}$ defined in \cref{e:step}. }}
%
\EndFor
\EndFor

\Statex

\For{$\ell = 1,2, \ldots, L$} \Comment{\hfill \cyan{// top-down sweep}}
\For{ $i =  n_\ell, \ldots, 2, 1$ } \Comment{\hfill \cyan{// reverse ordering}}
%
\State{ Read \emph{neighbors'} data $b(\N)$ for box $\B_i$:
\[
\begin{array}{ccr}
b(\R) \mathrel{-}= L_{\R}^{-1} X_{\R, \N} \, b(\N)
\end{array}
\]
} 
\Comment{\hfill \cyan{// $L_{\R}$ and $X_{\R, \N}$ defined in \cref{e:step}. }}
%
\State{ Update \emph{local} data $b(\R)$ and $b(\S)$ for box $\B_i$: 
\[
\begin{array}{ccr}
b(\R) & \mathrel{-}= & L_{\R}^{-1} X_{\R, \S} \, b(\S) \\
b(\R) & = & U_{\R}^{-1} \, b(\R) \\
b(\S) & \mathrel{-}= &  T \, b(\R) \\
\end{array}
\]
} 
\Comment{\hfill \cyan{// $\R, \S$ and $T$ defined in \cref{e:t}; $L_{\R}$, $U_{\R}$, and $X_{\R, \S}$ defined in \cref{e:step} }}

%
\EndFor
\EndFor

\end{algorithmic}
\end{algorithm}

